Glimpse: Enabling White-Box Methods to Use Proprietary Models for Zero-Shot LLM-Generated Text Detection

Advanced large language models (LLMs) can generate text almost indistinguishable from human-written text, highlighting the importance of LLM-generated text detection. However, current zero-shot techniques face challenges as white-box methods are restricted to use weaker open-source LLMs, and black-box methods are limited by partial observation from stronger proprietary LLMs. It seems impossible to enable white-box methods to use proprietary models because API-level access to the models neither provides full predictive distributions nor inner embeddings. To traverse the divide, we propose **Glimpse**, a probability distribution estimation approach, predicting the full distributions from partial observations. Despite the simplicity of Glimpse, we successfully extend white-box methods like Entropy, Rank, Log-Rank, and Fast-DetectGPT to latest proprietary models. Experiments show that Glimpse with Fast-DetectGPT and GPT-3.5 achieves an average AUROC of about 0.95 in five latest source models, improving the score by 51% relative to the remaining space of the open source baseline. It demonstrates that the latest LLMs can effectively detect their own outputs, suggesting that advanced LLMs may be the best shield against themselves. We release our code and data at https://github.com/baoguangsheng/glimpse.

==> figure/ablation_prompt.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={50pt 0pt 70pt 0pt},clip,width=1.0\linewidth]{source/ablation_prompt_barchart.pdf}   
    \caption{Ablation on prompt, evaluated on GPT-4 generations.}
    \label{fig:ablation_prompt}
\end{figure}

==> figure/ablation_topk.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={25pt 0pt 50pt 0pt},clip,width=0.5\linewidth]{source/ablation_topk_linechart.pdf}   
    \caption{Ablation on top-$K$, evaluated on GPT-4 generations. (\note{Need ablation on top-K on open-source LLMs, analyze the shift of curvature bring by estimation.})}
    \label{fig:ablation_topk}
\end{figure}

==> figure/ablation_vocab.tex <==
\begin{figure}
\vspace{-0.2in}
\begin{minipage}{0.49\linewidth}
    \centering
    \includegraphics[trim={10pt 10pt 30pt 0pt},clip,width=1.0\linewidth]{source/ablation_vocab_linechart.pdf}   
    \caption{Ablation on vocab size of ExFast-Detect, evaluated on GPT-4 generations. Overall geometric distribution shows stable performance on different size, while Zipfian distribution performs better with smaller size. }
    \label{fig:ablation_vocab}
\end{minipage}
\hfill\hspace{4pt}
\begin{minipage}{0.49\linewidth}
    \centering
    \includegraphics[trim={15pt 5pt 40pt 0pt},clip,width=1.0\linewidth]{source/auroc_curve_log.pdf}   
    \caption{ROC curves in log scale, where the {\color{red} red} line indicates a false alarm of 1\%. We draw the curves using a mixture of News, Story, and Tech. The dash lines denote the random classifier.}
    \label{fig:auroc_curve_log}
\end{minipage}        
\end{figure}



==> figure/distrib_over_rank.geometric.tex <==
\begin{figure}[t]
    % \vspace{-0.2in}
    \centering
    \includegraphics[trim={45pt 5pt 65pt 0pt},clip,width=1.0\linewidth]{source/distrib_over_rank.geometric.pdf}
    \caption{Probability distribution over ranks estimated by Geometric distribution.}
    \label{fig:distrib_over_rank.geometric}
\end{figure}

==> figure/distrib_over_rank.mlp.tex <==
\begin{figure}[t]
    % \vspace{-0.2in}
    \centering
    \includegraphics[trim={45pt 5pt 65pt 0pt},clip,width=1.0\linewidth]{source/distrib_over_rank.mlp.pdf}
    \caption{Probability distribution over ranks estimated by MLP distribution.}
    \label{fig:distrib_over_rank.mlp}
\end{figure}

==> figure/distrib_over_rank.zipfian.tex <==
\begin{figure}[t]
    % \vspace{-0.2in}
    \centering
    \includegraphics[trim={45pt 5pt 65pt 0pt},clip,width=1.0\linewidth]{source/distrib_over_rank.zipfian.pdf}
    \caption{Probability distribution over ranks estimated by Zipfian distribution.}
    \label{fig:distrib_over_rank.zipfian}
\end{figure}

==> figure/model_distributions.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{source/model_distributions.jpg}   
    \caption{Model distribution, decoding distribution, and samples.}
    \label{fig:model_distributions}
\end{figure*}

==> table/ablation_distrib.results.tex <==
\begin{table*}[t]
    \centering\scriptsize
    \begin{tabular}{l|cccc|cccc}
        \toprule
        \multirow{2}{*}{\bf Method (AUROC)} & \multicolumn{4}{c}{\bf ChatGPT} & \multicolumn{4}{c}{\bf GPT-4} \\
        & XSum & Writing & PubMed & Avg. & XSum & Writing & PubMed & Avg.  \\
        \midrule
        \multicolumn{9}{c}{\bf gpt-35-turbo-1106} \\
        ExEntropy(Geometric) & \bf 0.3124 & 0.0463 & \bf 0.1726 & 0.1771 & 0.6329 & 0.2722 & 0.2336 & 0.3795 \\
        ExEntropy(Zipfian) & 0.3119 & \bf 0.0522 & 0.1633 & 0.1758 & \bf 0.6386 & \bf 0.3055 & 0.2268 & \bf 0.3903 \\
        ExEntropy(MLP) & 0.3121 & 0.0489 & 0.1706 & \bf 0.1772 & 0.6352 & 0.2892 & \bf 0.2340 & 0.3861 \\
        \cdashline{1-9}
        ExRank(Geometric) & \bf 0.8584 & 0.\bf 9770 & \bf 0.7833 & \bf 0.8729 & \bf 0.6402 & \bf 0.8780 & \bf 0.7769 & \bf 0.7650 \\
        ExRank(Zipfian) & 0.6921 & 0.8633 & 0.6416 & 0.7324 & 0.6047 & 0.7867 & 0.6507 & 0.6807 \\
        ExRank(MLP) & 0.6982 & 0.8617 & 0.6246 & 0.7282 & 0.6064 & 0.8189 & 0.6339 & 0.6864 \\
        \cdashline{1-9}
        ExLogRank(Geometric) & 0.9280 & \bf 0.9933 & \bf 0.9504 & \bf 0.9572 & 0.6433 & 0.9411 & \bf 0.9076 & 0.8307 \\
        ExLogRank(Zipfian) & 0.9195 & 0.9929 & 0.9245 & 0.9456 & 0.6459 & \bf 0.9462 & 0.8910 & 0.8277 \\
        ExLogRank(MLP) & \bf 0.9326 & 0.9932 & 0.9399 & 0.9552 & \bf 0.6633 & \bf 0.9462 & 0.9067 & \bf 0.8387 \\
        \cdashline{1-9}
        ExFast(Geometric) & 0.9808 & \bf 0.9969 & \bf 0.9668 & \bf 0.9815 & 0.9095 & \bf 0.9966 & \bf 0.9441 & \bf 0.9500 \\
        ExFast(Zipfian) & 0.9780 & 0.9927 & 0.9320 & 0.9675 & \bf 0.9255 & 0.9920 & 0.9032 & 0.9402 \\
        ExFast(MLP) & \bf 0.9816 & 0.9951 & 0.9504 & 0.9757 & 0.9235 & 0.9953 & 0.9283 & 0.9490 \\
        \midrule
        \multicolumn{9}{c}{\bf gpt-4-1106} \\
        ExEntropy(Geometric) & \bf 0.4444 & 0.0273 & \bf 0.0982 & \bf 0.1900 & 0.5872 & 0.0954 & \bf 0.1133 & 0.2653 \\
        ExEntropy(Zipfian) & 0.4364 & \bf 0.0280 & 0.0904 & 0.1849 & \bf 0.5914 & \bf 0.1059 & 0.1078 & \bf 0.2684 \\
        ExEntropy(MLP) & 0.4395 & 0.0274 & 0.0930 & 0.1866 & 0.5896 & 0.0997 & 0.1079 & 0.2657 \\
        \cdashline{1-9}
        ExRank(Geometric) & \bf 0.8240 & \bf 0.9829 & \bf 0.8369 & \bf 0.8813 & \bf 0.7055 & \bf 0.9519 & \bf 0.8581 & \bf 0.8385 \\
        ExRank(Zipfian) & 0.6732 & 0.8843 & 0.6585 & 0.7387 & 0.6006 & 0.8435 & 0.7004 & 0.7148 \\
        ExRank(MLP) & 0.6740 & 0.8771 & 0.6277 & 0.7263 & 0.6406 & 0.8624 & 0.6487 & 0.7172 \\
        \cdashline{1-9}
        ExLogRank(Geometric) & 0.8348 & \bf 0.9917 & \bf 0.9638 & \bf 0.9301 & 0.7028 & 0.9805 & \bf 0.9650 & 0.8828 \\
        ExLogRank(Zipfian) & 0.8266 & 0.9915 & 0.9448 & 0.9210 & 0.6960 & \bf 0.9820 & 0.9521 & 0.8767 \\
        ExLogRank(MLP) & \bf 0.8413 & 0.9913 & 0.9538 & 0.9288 & \bf 0.7170 & \bf 0.9820 & 0.9540 & \bf 0.8843 \\
        \cdashline{1-9}
        ExFast(Geometric) & 0.9822 & \bf 0.9920 & \bf 0.9467 & \bf 0.9736 & 0.9716 & \bf 0.9887 & \bf 0.9437 & \bf 0.9680 \\
        ExFast(Zipfian) & 0.9821 & 0.9458 & 0.8925 & 0.9402 & 0.9819 & 0.9666 & 0.8857 & 0.9447 \\
        ExFast(MLP) & \bf 0.9856 & 0.9762 & 0.9156 & 0.9591 & \bf 0.9825 & 0.9804 & 0.9097 & 0.9576 \\
        \bottomrule
    \end{tabular}
    \caption{Ablation on distribution estimation techniques.}
    \label{tab:ablation_distrib.results}
\end{table*}




==> table/ablation_prompt.results.tex <==
\begin{table*}[t]
    \centering\small
    \begin{tabular}{llc@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c|c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c}
        \toprule
        \multirow{2}{*}{\bf Method} & \multirow{2}{*}{\bf Prompt} & \multicolumn{4}{c}{\bf GPT-3.5-Turbo} & \multicolumn{4}{|c}{\bf GPT-4} \\
        & & News & Story & Technical & Avg. & News & Story & Technical & Avg. \\
        \midrule
        babbage-002 & prompt0 & 0.9867 & 0.9921 & 0.9345 & 0.9711 & 0.8661 & 0.9268 & 0.8836 & 0.8921 \\
        babbage-002 & prompt1 & 0.9899 & \bf 0.9924 & 0.9372 & 0.9732 & 0.8882 & 0.9377 & 0.8841 & 0.9034 \\
        babbage-002 & prompt2 & 0.9920 & 0.9916 & 0.9543 & 0.9793 & 0.9054 & 0.9409 & 0.9152 & 0.9205 \\
        babbage-002 & prompt3 & \bf 0.9941 & \bf 0.9924 & \bf 0.9548 & \bf 0.9804 & \bf 0.9262 & \bf 0.9434 & \bf 0.9200 & \bf 0.9299 \\
        babbage-002 & prompt4 & 0.9932 & 0.9922 & 0.9542 & 0.9799 & 0.9141 & 0.9419 & 0.9192 & 0.9251 \\
        \midrule
        gpt-35-turbo-1106 & prompt0 & 0.9647 & 0.9770 & 0.8999 & 0.9472 & 0.8763 & 0.9734 & 0.8715 & 0.9071 \\
        gpt-35-turbo-1106 & prompt1 & \bf 0.9889 & 0.9849 & 0.9670 & 0.9803 & \bf 0.9461 & 0.9864 & \bf 0.9443 & \bf 0.9589 \\
        gpt-35-turbo-1106 & prompt2 & 0.9831 & \bf 0.9976 & \bf 0.9667 & \bf 0.9824 & 0.9235 & \bf 0.9984 & 0.9404 & 0.9541 \\
        gpt-35-turbo-1106 & prompt3 & 0.9837 & 0.9972 & 0.9656 & 0.9822 & 0.9230 & \bf 0.9984 & 0.9421 & 0.9545 \\
        gpt-35-turbo-1106 & prompt4 & 0.9807 & 0.9967 & 0.9616 & 0.9797 & 0.9129 & 0.9974 & 0.9428 & 0.9511 \\
        \midrule
        gpt-4-1106 & prompt0 & 0.6248 & 0.8648 & 0.8763 & 0.7886 & 0.5170 & 0.8686 & 0.8011 & 0.7289 \\
        gpt-4-1106 & prompt1 & 0.8161 & 0.9440 & 0.8799 & 0.8800 & 0.7164 & 0.9238 & 0.8316 & 0.8239 \\
        gpt-4-1106 & prompt2 & 0.9161 & 0.9315 & 0.8665 & 0.9047 & 0.8581 & 0.9245 & 0.8500 & 0.8775 \\
        gpt-4-1106 & prompt3 & 0.9663 & 0.9773 & 0.8994 & 0.9477 & 0.9460 & 0.9722 & 0.8840 & 0.9341 \\
        gpt-4-1106 & prompt4 & \bf 0.9838 & \bf 0.9912 & \bf 0.9453 & \bf 0.9734 & \bf 0.9691 & \bf 0.9879 & \bf 0.9475 & \bf 0.9682 \\
        \bottomrule
    \end{tabular}
    \caption{Ablation on prompt.}
    \label{tab:ablation_prompt.results}
\end{table*}

==> table/ablation_topk.results.tex <==
\begin{table*}[t]
    \centering\small
    \begin{tabular}{lcc@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c|c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c}
        \toprule
        \multirow{2}{*}{\bf Method (AUROC)} & \multirow{2}{*}{\bf Top-$K$}  & \multicolumn{4}{c}{\bf GPT-3.5-Turbo} & \multicolumn{4}{|c}{\bf GPT-4} \\
        & & News & Story & Technical & Avg. & News & Story & Technical & Avg. \\
        \midrule
        \multirow{3}{*}{Fast-Detect (GPT-3.5-Turbo)} 
        & top-$1$ & 0.9799 & \bf 0.9996 & \bf 0.9717 & \bf 0.9837 & 0.8694 & 0.9891 & 0.9427 & 0.9337 \\
        & top-$5$ & 0.9808 & 0.9971 & 0.9693 & 0.9824 & 0.9037 & 0.9958 & \bf 0.9470 & 0.9488 \\
        & top-$10$ & \bf 0.9837 & 0.9972 & 0.9656 & 0.9822 & \bf 0.9230 & \bf 0.9984 & 0.9421 & \bf 0.9545 \\
        \midrule
        \multirow{3}{*}{Fast-Detect (GPT-4)} 
        & top-$1$ & 0.9692 & \bf 0.9991 & \bf 0.9749 & \bf 0.9811 & 0.939 & \bf 0.9943 & \bf 0.9699 & 0.9677 \\
        & top-$5$ & 0.981 & 0.9951 & 0.9587 & 0.9783 & 0.9637 & 0.9916 & 0.9502 & \bf 0.9685 \\
        & top-$10$ & \bf 0.9838 & 0.9912 & 0.9453 & 0.9734 & \bf 0.9691 & 0.9879 & 0.9475 & 0.9682 \\
        \bottomrule
    \end{tabular}
    \caption{Ablation on top-K.}
    \label{tab:ablation_topk.results}
\end{table*}


==> table/intro_results.tex <==
\begin{table}[h]
    \centering\small
    \caption{Detection accuracy measured in AUROC across five latest LLMs, where the baseline Fast-DetectGPT uses an open-source model but our Glimpse uses a proprietary model. \revision{The methods are evaluated on the diverse Mix3 dataset, combining XSum, Writing, and PubMed, with details presented} in the main results (Table \ref{tab:main_results}). The notion ``{\it$\uparrow$}'' indicates the improvement relative to the remaining space, calculated by $(new - old) / (1.0 - old)$, following \cite{bao2023fast}.}
    % \vspace{-0.1in}
    \begin{tabular}{lccc@{\hspace{9pt}}ccc}
        \toprule
        \multirow{2}{*}{\bf Method} & \multirow{2}{*}{\bf ChatGPT} & \multirow{2}{*}{\bf GPT-4} & \multicolumn{2}{c}{\bf Claude-3} & \bf Gemini-1.5 & \multirow{2}{*}{\bf Avg.} \\
        &  &   & Sonnet & Opus & Pro \\    
        \midrule
         Fast-DetectGPT & \multirow{2}{*}{\revision{0.9487}} & \multirow{2}{*}{\revision{0.8999}} & \multirow{2}{*}{\revision{0.9260}} & \multirow{2}{*}{\revision{0.9468}} & \multirow{2}{*}{\revision{0.8072}} & \multirow{2}{*}{\revision{0.9057}} \\
         \emph{(Open-Source: GPT-Neo-2.7B)} & \\
         \midrule
         Glimpse (Fast-DetectGPT) & \revision{\bf 0.9766} & \revision{\bf 0.9411} & \revision{\bf 0.9576} & \revision{\bf 0.9689} & \revision{\bf 0.9244} & \revision{\bf 0.9537} \\
         \emph{(Proprietary: GPT-3.5)} & \bf ($\uparrow$ \revision{54}\%) & \bf ($\uparrow$ \revision{41}\%) & \bf ($\uparrow$ \revision{43}\%) & \bf ($\uparrow$ \revision{42}\%) & \bf ($\uparrow$ \revision{61}\%) & \bf ($\uparrow$ \revision{51}\%) \\
        \bottomrule
    \end{tabular}
    \label{tab:intro_results}
\end{table}



==> table/paraphrase_attack.tex <==
\begin{table*}[h]
    \centering\scriptsize
    \caption{Robustness under \emph{paraphrasing attack} with diverse lexicons and orders.}
    \begin{tabular}{l|cccc|cccc}
        \toprule
        \multirow{2}{*}{\bf Method} & \multicolumn{4}{c}{\bf ChatGPT + DIPPER (60 L)} & \multicolumn{4}{c}{\bf ChatGPT + DIPPER (60 O)} \\
        & XSum & Writing & PubMed & Avg. & XSum & Writing & PubMed & Avg. \\
        \midrule
        RoBERTa-base & 0.9498 & 0.8125 & 0.6504 & 0.8042 & 0.8847 & 0.6680 & 0.6147 & 0.7225 \\
        RoBERTa-large & 0.9264 & 0.7392 & 0.7019 & 0.7892 & 0.8850 & 0.6201 & 0.6736 & 0.7262 \\
        Fast-Detect (Neo-2.7) & \bf 0.9676 & \bf 0.9689 & 0.8623 & 0.9329 & 0.9744 & 0.9670 & 0.8531 & 0.9315 \\     
        Likelihood (GPT-3.5) & 0.4204 & 0.8065 & 0.8000 & 0.6756 & 0.7668 & 0.9797 & 0.8688 & 0.8718 \\
        \midrule
        \it PDE using Geometric \\
        \cindent Fast-Detect (Babbage) & 0.9589 & 0.9581 & \bf 0.9032 & \bf 0.9400 & \bf 0.9871 & 0.9810 & 0.9221 & \bf 0.9634 \\
        \cindent Fast-Detect (Davinci) & 0.9265 & 0.9526 & 0.8622 & 0.9138 &  0.9803 & 0.9931 & 0.8929 & 0.9555 \\
        \cindent Fast-Detect (GPT-3.5) & 0.8299 & 0.9439 & 0.8672 & 0.8803 &  0.9592 & \bf 0.9961 & \bf 0.9258 & 0.9604 \\
        % \cindent Fast-Detect (GPT-4) & 0.7527 & 0.8086 & 0.7720 & 0.7778 &   0.9276 & 0.9660 & 0.8886 & 0.9274 \\
        \it PDE using Zipfian and MLP \\
        \cindent Fast-Detect (GPT-3.5)$_{\text{Zipfian}}$ & 0.8429 & 0.9368 & 0.8562 & 0.8786 & 0.9658 & 0.9937 & 0.9155 & 0.9584 \\
        \cindent Fast-Detect (GPT-3.5)$_{\text{MLP}}$ & 0.8326 & 0.9360 & 0.8621 & 0.8769 & 0.9629 & 0.9945 & 0.9208 & 0.9594 \\
        \bottomrule
    \end{tabular}
    \label{tab:paraphrase_attack}
\end{table*}


